Efficient Hierarchical State Vector Simulation of Quantum Circuits via Acyclic Graph Partitioning

Early but promising results in quantum computing have been enabled by the concurrent development of quantum algorithms, devices, and materials. Classical simulation of quantum programs has enabled the design and analysis of algorithms and implementation strategies targeting current and anticipated quantum device architectures. In this paper, we present a graph-based approach to achieve efficient quantum circuit simulation. Our approach involves partitioning the graph representation of a given quantum circuit into acyclic sub-graphs/circuits that exhibit better data locality. Simulation of each sub-circuit is organized hierarchically, with the iterative construction and simulation of smaller state vectors, improving overall performance. Also, this partitioning reduces the number of passes through data, improving the total computation time. We present three partitioning strategies and observe that acyclic graph partitioning typically results in the best time-to-solution. In contrast, other strategies reduce the partitioning time at the expense of potentially increased simulation times. Experimental evaluation demonstrates the effectiveness of our approach.

==> related_work.tex <==
\section{Related work}
\label{sec:related}

There are many recent quantum simulation systems. 


Intel's $q$H$i$PSTER~\cite{} is a specialized distributed quantum simulation environment that reached to computation of up to 42 qubits through better algorithm design and hardware specific optimizations on the Stampede supercomputer.

QX~\cite{} is quantum simulation platform which defines its own low-level language to implement quantum operations. It exploits several hardware optimizations, efficient computation and scheduling techniques to improve its performance.

H\"aner et al.~\cite{haner-petabyte} focus on improving the performance and memory requirements of quantum supremacy circuits.
Wu et al.~\cite{}'s recent work explores data compression techniques.
Our technique is orthogonal to the improvements in these work, meaning that they can be applied in addition to our approach as well.

Intel IQS, recent work of Intel, is the new version $q$H$i$PSTER, which is one of the few open source simulations. We compare our approach with IQS as this is the state-of-the-art technique.

Our approach explores a unique approach that can benefit from the optimizations they apply as well...
